On Empirical Risk Minimization with Dependent and Heavy-Tailed Data

In this work, we establish risk bounds for the Empirical Risk Minimization (ERM) with both dependent and heavy-tailed data-generating processes. We do so by extending the seminal works of Mendelson [Men15, Men18] on the analysis of ERM with heavy-tailed but independent and identically distributed observations, to the strictly stationary exponentially $\beta$-mixing case. Our analysis is based on explicitly controlling the multiplier process arising from the interaction between the noise and the function evaluations on inputs. It allows for the interaction to be even polynomially heavy-tailed, which covers a significantly large class of heavy-tailed models beyond what is analyzed in the learning theory literature. We illustrate our results by deriving rates of convergence for the high-dimensional linear regression problem with dependent and heavy-tailed data.

==> poly_ex_diequaltod.tex <==
\subsection{Example 2}\label{sec:examplepoly}
Let $\tilde{X}_{t,i}$ denote the $i$-th coordinate of the vector $\tilde{X}_t\in\mathbb{R}^d$. Consider the following process: for $i=1,2,\cdots,d$, $\eta_3> 2+2\iota$, where $\iota>0$ is a small number, and $t=0,1,\cdots$  \cite{pillai1991semi}:
\[   
\tilde{X}_{t,i} = 
\begin{cases}
	2^\frac{1}{\eta_3}\tilde{X}_{t-1,i} &\quad\text{with probability  }1/2\\
	\min\left(2^\frac{1}{\eta_3}\tilde{X}_{t-1,i},\delta_{t,i}\right)&\quad\text{with probability  }1/2\numberthis\label{eq:arsp}
\end{cases}
\]
where $\{\delta_{t,i}\}_{i=1,2,\cdots,d, t=1,2,\cdots}$ be $\iid$ Pareto random variables with the distribution
\begin{align}
	L_+(\delta;\eta_3,d)=\frac{\eta_3(d\delta)^{\eta_3-1}}{\left(1+(d\delta)^{\eta_3}\right)^2} \quad \delta>0, \eta_3>2+2\iota
\end{align}
and we write $X\sim L_+(\eta,\sigma)$ to denote that $X$ is a Pareto random variable with parameters $\eta$ and $\sigma$. The survival function of $\delta\sim L_+(\eta_3,d)$ is given by, for any $t>0$
\begin{align}
	\mathbb{P}(\delta>t)=(1+(dt)^{\eta_3})^{-1}
\end{align}	
	\cite{pillai1991semi} shows that the AR(1) process given by \eqref{eq:arsp} is strictly stationary if $\tilde{X}_{0,i}\sim L_+(\eta_3,d)$, and $\tilde{X}_{0,i}$ are independent of each other for $i=1,2,\cdots,d$. The stationary distribution is given by $L_+(\eta_3,d)$. 
	Let $\tilde{X}_{1,t}$ and $\tilde{X}_{2,t}$ be two independent trails of the process in \eqref{eq:arsp}. Let $\{U_t\}_{t=0,1,\cdots}$ be a sequence of $\iid$ $U[0,1]$ random variables. Now consider the process 
	\[   
	{X}_{t,i} = 
	\begin{cases}
		\tilde{X}_{1,t,i} &\quad\text{if }U_t\leq 1/2\\
		-\tilde{X}_{2,t,i}&\quad\text{if }U_t>1/2\numberthis\label{eq:arsp12}
	\end{cases}
	\]
	Let $\pi(X_{t_1},X_{t_2},\cdots,X_{t_n})$ be the joint distribution of $X_{t_1},X_{t_2},\cdots,X_{t_n}$ for a set of time points $t_1,t_2,\cdots,t_n$. Now for any positive integer $k$, 
	\begin{align*}
		&\pi(\{X_{t_i+k}\}_{i=1}^n)
		=\pi(\{\tilde{X}_{1,t_i+k}\mathbbm{1}(U_{t_i+k}\leq 1/2)-\tilde{X}_{2,t_i+k}\mathbbm{1}(U_{t_i+k}> 1/2)\}_{i=1}^n)\\
		=&\pi(\{\tilde{X}_{1,t_i}\mathbbm{1}(U_{t_i}\leq 1/2)-\tilde{X}_{2,t_i}\mathbbm{1}(U_{t_i}> 1/2)\}_{i=1}^n)
		=\pi(\{X_{t_i}\}_{i=1}^n)   \numberthis\label{eq:}
	\end{align*}
The second equality above follows from the fact $\tilde{X}_{1,t}$ and $\tilde{X}_{2,t}$ are strictly stationary process and $\{U_t\}$ is $\iid$. So $X_t$ is a strictly stationary process with marginal distribution of $X_{t,i}$ given by symmetric Pareto distribution
\begin{align}
	L(x;\eta_3,d)=\frac{\eta_3(d|\delta|)^{\eta_3-1}}{2\left(1+(d|\delta|)^{\eta_3}\right)^2} \quad -\infty<\delta<\infty, \eta_3>2+2\iota.
\end{align} 
	 It is shown in Lemma 1 of \cite{ristic2008generalized}, that the AR(1) process in \eqref{eq:arsp} is $\phi$-mixing with 
	\begin{align}
		\phi(k)=k\log 2/(2^k-1)  \qquad k=1,2,\cdots
	\end{align}
where $\phi$-mixing coefficients are defined as in \cite{bradley2005basic}. We also have 
\begin{align}
	\beta(k)\leq \phi(k)\leq \frac{k\log 2}{2^k-1} \leq e^{-\frac{k}{3}}.
\end{align}
Since $X_t$ depends only on $X_{1,t}$, $X_{2,t}$, and $U_t$, $X_{1,t}$, and $X_{2,t}$ are independent and exponentially $\beta$-mixing, and $U_t$ is $\iid$, $X_t$ is also exponentially $\beta$-mixing. Let $\{Y_i\}_{i\in\mathbb{Z^+}}$, $Y_i\in\mathbb{R}$ denote the sequence given by $Y_i={\theta^*}^\top X_i+\upsilon_i$, where $\theta^*\in B_1^d(R)$, as before. Let $\{\upsilon_i\}_{i=1}^n$ be independent of $X_i$ $\forall i$ and be an $\iid$ sequence of $0$ mean random variables with heavy tails such that for all $t>0$, 
\begin{align*}
\mathbb{P}\left(|\upsilon_{i}|\geq t\right)\leq 1/(1+t^{\eta_4}) \qquad \eta_4>2+2\iota.
\end{align*} 
Like in Example~\ref{sec:ex1}, we consider LS-ERM with the function class given by 
\begin{align}
	\mathcal{F}\coloneqq \cF_R=\left\lbrace\langle\theta,\cdot\rangle:\theta\in B_1^d(R)\right\rbrace,\label{eq:fclasswei}
\end{align}
where $B_1^d(R)$ denotes the $d$-dimensional $\ell_1$-ball with radius $R$.
We denote the difference function class $\cF_R-\cF_R$ by $\cH_R$. Let us first verify the assumptions for this setting:
\begin{itemize}
	\item Since $Y_i$ depends only on $X_i$, and $\upsilon_i$ are $\iid$, $\{(X_i,Y_i)\}$ is a strictly stationary $\beta$-mixing sequence with $\beta(k)\leq e^{-k/3}$. This proves that condition (1) of Assumption~\ref{as:datagenprocess} is true for this probelm. 
	\item Now we will verify condition (2) of Assumption~\ref{as:datagenprocess}. Let $\sigma_{X,p}$ denote $\|X\|_p$ for $p>0$. Then
	\begin{align}
		\expec{\left(\theta^\top X\right)^2}{}=\sum_{i=1}^{d}\frac{\theta_i^2\sigma_{X_i,2}^2}{d}\geq \frac{\sigma_0^2}{d}\|\theta\|_2^2
	\end{align}
where $\sigma_0=\sigma_{X_i,2}$ for all $i=1,2,\cdots,d$.
	Since $X_i\sim L(\eta_3)$, for any $\theta_i\in \mathbb{R}$ we have
	\begin{align}
		\|\theta_iX_i\|_{\eta_3-0.5\iota}\leq K_1|\theta_i|\sigma_{X,\eta_3-0.5\iota}
	\end{align}
	So,
	\begin{align}
		\|\theta^\top X\|_{\eta_3-0.5\iota}\leq K_1\|\theta\|_1\sigma_{X,\eta_3-0.5\iota}\leq\frac{K_1\sqrt{d}\|\theta\|_1\sigma_{X,\eta_3-0.5\iota}}{\sigma_0\|\theta\|_2}\|\theta^\top X\|_2\leq \frac{K_1d\sigma_{X,\eta_3-0.5\iota}}{\sigma_0}\|\theta^\top X\|_2\
	\end{align}
	Then from Lemma 4.1 of \cite{pmlr-v35-mendelson14} we have that the condition (2) of Assumption~\ref{as:datagenprocess} is true here. 
	\item Since $\upsilon_i$ and $X_i$ are independent, and $\expec{\upsilon_{i}}{}=0$, we have $\expec{\upsilon_it^\top X_i}{}=0$. Let $\eta_2=\min(\eta_3,\eta_4)$. Then using Markov's inequality, for any $t\in\cH_R$ and $\forall i$, we have,
	\begin{align*}
		&\mathbb{P}\left(\abs{\upsilon_it^\top X_i-\expec{\upsilon_it^\top X_i}{}}\geq \tau\right)
		=	\mathbb{P}\left(\abs{\upsilon_it^\top X_i}\geq \tau\right)
		\leq  \frac{\|\upsilon_it^\top X_i\|_{\eta_2}^{\eta_2}}{\tau^{\eta_2}}\\
		\leq & \frac{\|\upsilon_i\|_{\eta_2}^{\eta_2}\left(\sum_{j=1}^d\|t_j X_{i,j}\|_{\eta_2}\right)^{\eta_2}}{\tau^{\eta_2}}
		\leq \frac{\left(R\sigma_\upsilon\sigma_{X,\eta_2}\right)^{\eta_2}}{\tau^{\eta_2}} 
	\end{align*}
	where for all $i,j$, $\|\upsilon_i\|_{\eta_2}=\sigma_\upsilon$, and $\|X_{i,j}\|_{\eta_2}=\sigma_{X,\eta_2}/d$. This implies that condition (3b) of Assumption~\ref{as:datagenprocess} is true in this setting.
\end{itemize}
 We need the following two lemmas to establish a bound on $\omega_\mu(\cF_R-\cF_R,\tau Q_{\cH_R}(2\tau)/16)$ in Proposition~\ref{prop:paretorate}. We provide the proofs of the lemma in Appendix. 
\begin{lemma}\label{lm:w1starconc}
	Let $\{X'_i\}_{i=1}^\mu$ be an $\iid$ sample from $L(\eta_3,d)$ and let $w$ be a random vector where coordinates of $w$ are given by
	\begin{align*}
		w_j=\frac{1}{\sqrt{\mu}}\sum_{i=1}^\mu X'_{i,j} \qquad j=1,2,\cdots,d \numberthis\label{eq:wjdefpoly}
	\end{align*}
Then we have
	\begin{align*}
		\mathbb{P}\left(\abs{w_j}\geq t\right)\leq C_3\left(d^{\eta_3-2p-1}\mu^{1-\frac{\eta_3}{2}}t^{\eta_3-2p}+d^{-2}t^{-p}\right) \numberthis\label{eq:w1starconc}
	\end{align*}
	for some constant $C_3>0$.
\end{lemma}
Let $\{w_j^*\}_{j=1}^d$ be the non-increasing arrangement of $\{|w_j|\}_{j=1}^d$. 
\begin{lemma}\label{lm:expecwstarsumpoly}
	Let $w_1,w_2,\cdots,w_d$ are independent copies of a random variable such that \eqref{eq:w1starconc} is true for all $j=1,2,\cdots,d$, i.e., 
	\begin{align*}
		\mathbb{P}\left(\abs{w_j}\geq t\right)\leq C_3\left(d^{\eta_3-2p-1}\mu^{1-\frac{\eta_3}{2}}t^{\eta_3-2p}+d^{-2}t^{-p}\right) \quad j=1,2,\cdots,d
	\end{align*}
	for $\eta_3>2+2\iota$, and $p=\eta_2-0.5\iota$. Then for every $1\leq k\leq d$,
	\begin{align*}
		\expec{\left(\sum_{i=1}^k{w_i^*}^2\right)^\frac{1}{2}}{}\leq  C_6\sqrt{k}\left(d^{\eta_3/2-p-\eta_3/(2p)+1-1/p}\mu^{1/2-\eta_3/4}+d^{-1/p}\right) 
	\end{align*}
	for some constant $C_6>0$ which depends on $\eta_3$ and $p$.
\end{lemma}
\iffalse
\begin{proof}
	Consider the one-to-one transformation of $w_j$, $z_j=((dw_j)^{\eta_3}+1)^{1/\eta_3}$. The distribution function of $z_j$ is given by 
	\begin{align*}
		\mathbb{P}(z_j\leq t)=1-t^{-\eta_3} \qquad t>1
	\end{align*} 
Then, using Jensen's inequality we have
\begin{align}
	\expec{{z_j^*}^2}{}=\expec{((dw_j^*)^{\eta_3}+1)^{2/\eta_3}}{}\geq \expec{\frac{(dw_j^*)^2+1}{2}}{} \label{eq:wzmomentrel}
\end{align} 
From \cite{huang1975note}, we have for $j\geq 1$
\begin{align}
	\expec{{z_j^*}^2}{}=\frac{d!\Gamma\left(j-2/\eta_3\right)}{(j-1)!\Gamma\left(d+1-2/\eta_3\right)}=\frac{d!\Gamma\left(j-2/\eta_3\right)}{(j-1)!\Gamma\left(1-2/\eta_3\right)\Pi_{i=1}^{d}\left(i-2/\eta_3\right)}
\end{align}  
For $j=1$, 
\begin{align}
	\expec{{z_j^*}^2}{}=\frac{1}{\Pi_{i=1}^{d}\left(1-2/(i\eta_3)\right)}=\Pi_{i=1}^{d}\left(1+\frac{2}{i\eta_3-2}\right)\leq \exp\left(\sum_{i=1}^d\frac{2}{i\eta_3-2}\right)\leq \left(\frac{d+1-2/\eta_3}{1-2/\eta_3}\right)^\frac{2}{\eta_3}
\end{align} 
For $j\geq 2$, using $1+x\leq e^x$
\begin{align}
	\expec{{z_j^*}^2}{}=\frac{\Pi_{i=1}^{j-1}\left(1-2/(i\eta_3)\right)}{\Pi_{i=1}^{d}\left(1-2/(i\eta_3)\right)}\leq \exp\left(\sum_{i=1}^d\frac{2}{i\eta_3-2}-\sum_{i=1}^{j-1}\frac{2}{i\eta_3}\right)\leq \left(\frac{d+1-2/\eta_3}{(1-2/\eta_3)(j-1)}\right)^\frac{2}{\eta_3}
\end{align}   
So for any $k\geq 2$, we have
\begin{align*}
	\sum_{j=1}^k \expec{{z_j^*}^2}{}\leq \left(\frac{d+1-2/\eta_3}{1-2/\eta_3}\right)^\frac{2}{\eta_3}\left(1+\frac{k^{1-2/\eta_3}}{1-2/\eta_3}\right)
\end{align*}
Using \eqref{eq:wzmomentrel} we get
\begin{align*}
	\sum_{j=1}^k \expec{{w_j^*}^2}{}\leq \left(\frac{d+1-2/\eta_3}{1-2/\eta_3}\right)^\frac{2}{\eta_3}\frac{(2+6k^{1-2/\eta_3})}{d^2}
\end{align*}
Using Jensen's inequality,
\begin{align}
	\expec{\left(\sum_{j=1}^k {w_j^*}^2\right)^\frac{1}{2}}{}\leq \left(\sum_{j=1}^k \expec{{w_j^*}^2}{}\right)^\frac{1}{2}\leq \left(\frac{d+1-2/\eta_3}{1-2/\eta_3}\right)^\frac{1}{\eta_3}\frac{(2+3k^{1/2-1/\eta_3})}{d}\leq \frac{K_2k^{1/2-1/\eta_3}}{d^{1-1/\eta_3}}
\end{align}
for some constant $K_2>0$ which depends on $\eta_3$.
\end{proof}
\fi
\begin{proposition}\label{prop:paretorate}
	Consider the learning problem described in the beginning of Section~\ref{sec:examplepoly}. Then with probability at least \eqref{eq:thm10probpoly}, we have,
	\begin{align*}
		\|\hat{f}-f^*\|_{L_2} \leq \max\left\{N^{-\frac{1}{4}\left(1-\frac{1}{\eta_2}\right)+\iota},\frac{C_9R}{\tau Q_{\cH_R}(2\tau)^{3/2}}d^{-1/p}N^{-1/2+\iota}\right\} \numberthis\label{eq:errorboundalphapareto}
	\end{align*}
\end{proposition}
\begin{proof}[Proof of Proposition~\ref{prop:paretorate}]
\textbf{Bound on $\omega_\mu(\cF_R-\cF_R,\tau Q_{\cH_R}(2\tau)/16)$:}
	\begin{align}
		&\expec{\sup_{f\in\cF_R\cap s\mathcal{D}_{f^*}}\abs{\frac{1}{\sqrt{\mu}}\sum_{i=1}^\mu\epsilon_i(f-f^*)(X'_i)}}{}\leq \expec{\sup_{t\in B_1^d(2R)\cap B_2^d(s)}\left\langle\frac{1}{\sqrt{\mu}}\sum_{i=1}^\mu X'_i,t\right\rangle}{}\\
		=&\expec{\sup_{t\in B_1^d(2R)\cap B_2^d(s)}\left\langle w,t\right\rangle}{}
		\expec{\sup_{t\in B_1^d(2R)\cap B_2^d(s)}w^\top t}{}=s\expec{\sup_{t\in B_1^d(2R/s)\cap B_2^d(1)}w^\top t}{}\\
		\leq& 2s\expec{\left(\sum_{j=1}^{(2R/s)^2} {w_j^*}^2\right)^\frac{1}{2}}{}
	\end{align}
If $(2R/s)^2<d$, using Lemma~\ref{lm:expecwstarsumpoly} we get
\begin{align}
	\expec{\sup_{t\in B_1^d(2R)\cap B_2^d(s)}w^\top t}{}\leq 4C_6R\left(d^{\eta_3/2-p-\eta_3/(2p)+1-1/p}\mu^{1/2-\eta_3/4}+d^{-1/p}\right) \leq C_7Rd^{-1/p}
\end{align}
for some constant $C_7>0$.\\
If $(2R/s)^2\geq d$,
\begin{align}
	\expec{\sup_{t\in B_1^d(2R)\cap B_2^d(s)}w^\top t}{}\leq 2s\sigma_{X,2}d^{-1/2} 
\end{align}
So when $(2R/s)^2\geq d$, 
\begin{align*}
	\expec{\sup_{f\in\cF_R\cap s\mathcal{D}_{f^*}}\abs{\frac{1}{\mu}\sum_{i=1}^\mu\epsilon_i(f-f^*)(X'_i)}}{}\leq \gamma s\numberthis\label{eq:omegamucond}
\end{align*} for all $s>0$. When $\mu\leq C_8d^{1-2/p}$, we have $(2R/s)\leq \sqrt{d}$ for
\begin{align*}
	s\geq \frac{C_7Rd^{-1/p}}{\gamma\sqrt{\mu}}
\end{align*}
When $\mu> C_8d^{1-2/p}$, we have $(2R/s)\geq \sqrt{d}$ for
\begin{align*}
	s\leq \frac{C_7Rd^{-1/p}}{\gamma\sqrt{\mu}}
\end{align*}
Combining the above facts, and choosing $\mu=\frac{N^rQ_\cH(2\tau)c^\frac{1}{\eta_1}}{4}$, and $r=1-2\iota$ we get
\[
\omega_\mu(\cF_R-\cF_R,\tau Q_{\cH_R}(2\tau)/16)\leq 
\begin{cases}
	\frac{C_9R}{\tau Q_{\cH_R}(2\tau)^{3/2}}d^{-1/p}N^{-1/2+\iota} & \text{if $\mu\leq C_8d^{1-2/p}$} \\
	0 & \text{if $\mu> C_8d^{1-2/p}$}. 
\end{cases} \numberthis\label{eq:omegaboundweipoly}
\]
where $C_9=32C_7/c^{1/(2\eta_1)}$. Then using part 2 of Theorem~\ref{th:mainthm2}, we get, 
\begin{align*}
	\|\hat{f}-f^*\|_{L_2} \leq \max\left\{N^{-\frac{1}{4}\left(1-\frac{1}{\eta_2}\right)+\iota},\frac{C_9R}{\tau Q_{\cH_R}(2\tau)^{3/2}}d^{-1/p}N^{-1/2+\iota}\right\} 
\end{align*}
with probability given by at least \eqref{eq:thm10probpoly}.
\end{proof}

==> section3.tex <==

\iffalse
{\color{blue}\textbf{Note:} It would be ideal if we could assume a lower bound on the tail of $\xi_1X_1$ and then show that \eqref{eq:sumheavyconc} holds instead of assuming \eqref{eq:sumheavyconc}. For that, we need to establish lower bound on the tail probability of the sum of $\iid$ variables from the lower bound on the tail probability of the random variable. Couln't find anything suitable.}\\
\begin{align}
	\kappa_N(s)=\sup_{f\in\cF\cap s\cD_{f^*}}\abs{\frac{1}{\sqrt{N}}\sum_{i=1}^N\epsilon_i\xi_i(f-f^*)(X_i)}
\end{align}
Let,
\begin{align*}
	\alpha_N^*(\gamma,\delta)=\inf\{s>0:\pro\left(\kappa_N(s)\leq \gamma s^2\sqrt{N}\right)\geq 1-\delta\}
\end{align*}
\begin{theorem} \label{th:mainthm1}
	Let $\cF \subset L_2(\pi)$ be a closed, convex class of functions. Let Assumptions~\ref{as:betamix}-\ref{as:etacon} hold. Then with probability at least $\mathscr{P}$, we have
	\begin{align*}
		\|\hat{f}-f^*\|_{L_2}\leq \omega_\mu(\cF-\cF,\tau Q_{\cF-\cF}(2\tau)/16) \numberthis\label{eq:errorbound}
	\end{align*}
where, 
\begin{align*}
	\mathscr{P}=&1-2\exp\left(-\frac{NQ_\cH(2\tau)^3}{2(4-Q_\cH(2\tau))^2}\left(\frac{c}{\mathscr{G}(N)}\right)^\frac{1}{\eta_1}\right)-\frac{NQ_\cH(2\tau)c^\frac{1}{\eta_1}}{4\mathscr{G}(N)^\frac{1}{\eta_1}}\exp(-\mathscr{G}(N))\\
	-&N\exp\left(-\frac{(N\tau^*)^\eta}{C_1}\right)-\exp\left(-\frac{N^2{\tau^*}^2}{C_2(1+NV)}\right)-\exp\left(-\frac{N{\tau^*}^2}{C_3}\exp\left(\frac{(N\tau^*)^{\eta(1-\eta)}}{C_4(\log (N\tau^*))^\eta}\right)\right),\numberthis\label{eq:mathscrP} \\
   \mu=&\frac{NQ_\cH(2\tau)c^\frac{1}{\eta_1}}{4\mathscr{G}(N)^\frac{1}{\eta_1}} \quad \tau^*=\frac{\tau^2\omega_\mu^2(\cH,\tau Q_{\cF-\cF}(2\tau)/16)Q_\cH(2\tau)}{16}.\numberthis\label{eq:mutau0choice}
\end{align*}
\end{theorem}
\begin{proof}[of~\ref{th:mainthm1}]
	We will denote the class $\cF-f^*$ by $\cH$. From Lemma~\ref{lm:thilowbound} it follows that if $\rho>\omega_\mu(\cH,\tau Q_{\cF-\cF}(2\tau)/16)$, then with probability at least $\mathscr{P}_1=1-2\exp\left(-\frac{NQ_\cH(2\tau)^3}{2(4-Q_\cH(2\tau))^2}\left(\frac{c}{\mathscr{G}(N)}\right)^\frac{1}{\eta_1}\right)-\frac{NQ_\cH(2\tau)c^\frac{1}{\eta_1}}{4\mathscr{G}(N)^\frac{1}{\eta_1}}\exp(-\mathscr{G}(N))$, for every $f\in \cF$ that satisfies $\|f-f^*\|_{L_2}\geq \rho$, 
	\begin{align}
		\frac{1}{N}\sum_{i=1}^N(f-f^*)^2(X_i)\geq \frac{\tau^2\|f-f^*\|^2_{L_2}Q_\cH(2\tau)}{4}
	\end{align}
So, with probability at least $\mathscr{P}_1$, for every $f\in \cF$ that satisfies $\|f-f^*\|_{L_2}\geq \rho$,
\begin{align*}
	P_N\mathcal{L}_f\geq2\left( \frac{1}{N}\sum_{i=1}^N\xi_i(f-f^*)(X_i)-\expec{\xi(f-f^*)}{}\right)+\frac{\tau^2\|f-f^*\|^2_{L_2}Q_\cH(2\tau)}{4} \numberthis\label{eq:PnLfintermedbound}
\end{align*}
\iffalse
Say $\alpha_N^*(\gamma,\delta/4)=\alpha_N$. If $\|f-f^*\|_{L_2}\leq\alpha_N$ then
\begin{align}
	\pro\left(\abs{\frac{1}{N}\sum_{i=1}^N\epsilon_i\xi_i(f-f^*)(X_i)}\leq \gamma \alpha_N^2\right)\geq 1-\frac{\delta}{4}
\end{align} 

Now,
\begin{align*}
	&\pro\left(\abs{\frac{1}{N}\sum_{i=1}^N\epsilon_i\xi_i(f-f^*)(X_i)}\leq \gamma \alpha_N^2\right)\\
	\leq &\pro\left(\abs{\frac{1}{N}\sum_{i=1}^\mu\sum_{j=(i-1)(a+b)+1}^{(i-1)(a+b)+a}\epsilon_j\xi_j(f-f^*)(X_j)}\leq \gamma \alpha_N^2+\abs{\frac{1}{N}\sum_{i=1}^\mu\sum_{j=(i-1)(a+b)+a+1}^{(a+b)i}\epsilon_j\xi_j(f-f^*)(X_j)}\right)\\
	\leq &\pro\left(\abs{\frac{1}{N}\sum_{i=1}^\mu\sum_{j=(i-1)(a+b)+1}^{(i-1)(a+b)+a}\epsilon_j\xi_j(f-f^*)(X_j)}\leq \gamma \alpha_N^2+\frac{1}{N}\sum_{i=1}^\mu\sum_{j=(i-1)(a+b)+a+1}^{(a+b)i}\abs{\xi_j(f-f^*)(X_j)}\right)\\
	\leq &\pro\left(\abs{\frac{1}{N}\sum_{i=1}^\mu\sum_{j=(i-1)(a+b)+1}^{(i-1)(a+b)+a}\epsilon_j\xi_j(f-f^*)(X_j)}\leq \gamma \alpha_N^2+\frac{b\mu}{N}\sup_{j\in\{1,2,\cdots,n\} }\abs{\xi_j(f-f^*)(X_j)}\right)\\
	\leq &\pro\left(\abs{\frac{1}{N}\sum_{i=1}^\mu\sum_{j=(i-1)(a+b)+1}^{(i-1)(a+b)+a}\epsilon_j\xi_j(f-f^*)(X_j)}\leq \gamma \alpha_N^2+\frac{b\mu}{N}\sup_{j\in\{1,2,\cdots,n\} }\abs{\xi_j(f-f^*)(X_j)}\given\right.\\
	&\left.\sup_{j\in\{1,2,\cdots,n\} }\abs{\xi_j(f-f^*)(X_j)}\leq B\right)
	+\pro\left(\sup_{j\in\{1,2,\cdots,n\} }\abs{\xi_j(f-f^*)(X_j)}\geq B\right)\\
	\leq & \pro\left(\abs{\frac{1}{N}\sum_{i=1}^\mu\sum_{j=(i-1)(a+b)+1}^{(i-1)(a+b)+a}\epsilon_j\xi_j(f-f^*)(X_j)}\leq \gamma \alpha_N^2+\frac{Bb\mu}{N}\given\sup_{j\in\{1,2,\cdots,n\} }\abs{\xi_j(f-f^*)(X_j)}\leq B\right)
	+p(B)\\
	=& \expec{\mathbbm{1} \left(\abs{\frac{1}{N}\sum_{i=1}^\mu\sum_{j=(i-1)(a+b)+1}^{(i-1)(a+b)+a}\epsilon_j\xi_j(f-f^*)(X_j)}\leq \gamma \alpha_N^2+\frac{Bb\mu}{N}\right)\given\sup_{j\in\{1,2,\cdots,n\} }\abs{\xi_j(f-f^*)(X_j)}\leq B}{}
	+p(B)\\
	\stackrel{(1)}{\leq}& \expec{\mathbbm{1} \left(\abs{\frac{1}{N}\sum_{i=1}^\mu\sum_{j=(i-1)(a+b)+1}^{(i-1)(a+b)+a}\tilde{\epsilon}_j\tilde{\xi}_j(f-f^*)(\tilde{X}_j)}\leq \gamma \alpha_N^2+\frac{Bb\mu}{N}\right)\given\sup_{j\in\{1,2,\cdots,n\} }\abs{\xi_j(f-f^*)(X_j)}\leq B}{}\\
	+&p(B)+(b-1)\beta(b)\\
	\leq & \expec{\mathbbm{1} \left(\abs{\sum_{i=1}^a\sum_{j=1}^{\mu}\tilde{\epsilon}_{(j-1)(a+b)+i}\tilde{\xi}_{(j-1)(a+b)+i}(f-f^*)(\tilde{X}_{(j-1)(a+b)+i})}\leq \gamma N \alpha_N^2+Bb\mu\right)\given\sup_{j\in\{1,2,\cdots,n\} }\abs{\xi_j(f-f^*)(X_j)}\leq B}{}\\
	+&p(B)+(b-1)\beta(b)
\end{align*}
\fi
Under Assumption~\ref{as:betamix}-\ref{as:etacon}, using Lemma~\ref{lm:rio}, we get
\begin{align*}
	&\pro\left(\abs{\frac{1}{N}\sum_{i=1}^N\xi_i(f-f^*)(X_i)-\expec{\xi(f-f^*)}{}}\geq \tau_0\right)\\
	\leq& N\exp\left(-\frac{(N\tau_0)^\eta}{C_1}\right)+\exp\left(-\frac{N^2\tau_0^2}{C_2(1+NV)}\right)+\exp\left(-\frac{N\tau_0^2}{C_3}\exp\left(\frac{(N\tau_0)^{\eta(1-\eta)}}{C_4(\log (N\tau_0))^\eta}\right)\right)\equiv \mathscr{P}_2 \numberthis\label{eq:noiseconc}
\end{align*}
where $$V\leq \expec{\left(\xi_1(f-f^*)(X_1)\right)^2}{}+4\sum_{i\geq 0}\expec{B_i\left(\xi_1(f-f^*)(X_1)\right)^2}{}.$$
$\{B_i\}$ is some sequence such that $B_i\in[0,1]$, and  $\expec{B_i}{}\leq \beta(i)$. $C_1,C_2,C_3$ are constants which depend on $c,\eta,\eta_1,\eta_2$. Observe that,
\begin{align*}
	V\leq& \expec{\left(\xi_1(f-f^*)(X_1)\right)^2}{}+4\sum_{i\geq 0}\expec{B_i\left(\xi_1(f-f^*)(X_1)\right)^2}{}\\
	\leq & \expec{\left(\xi_1(f-f^*)(X_1)\right)^2}{}+4\sum_{i\geq 0}\sqrt{\expec{B_i^2}{}\expec{\left(\xi_1(f-f^*)(X_1)\right)^4}{}}\\
	\leq & \expec{\left(\xi_1(f-f^*)(X_1)\right)^2}{}+4\expec{\left(\xi_1(f-f^*)(X_1)\right)^4}{}\sum_{i\geq 0}\sqrt{\expec{B_i}{}}\\
	\leq & \expec{\left(\xi_1(f-f^*)(X_1)\right)^2}{}+4\expec{\left(\xi_1(f-f^*)(X_1)\right)^4}{}\sum_{i\geq 0}\sqrt{\beta(i)}\\
	\leq & \expec{\left(\xi_1(f-f^*)(X_1)\right)^2}{}+4\expec{\left(\xi_1(f-f^*)(X_1)\right)^4}{}\sum_{i\geq 0}\exp(-ci^{\eta_1}/2)\leq C
\end{align*}
\iffalse
\begin{align*}
	&\pro\left(\abs{\frac{1}{N}\sum_{i=1}^N\xi_i(f-f^*)(X_i)-\expec{\xi(f-f^*)}{}}\leq \tau_0\right)
	\leq& \pro\left(\abs{\frac{1}{N}\sum_{i=1}^N\xi_i(f-f^*)(X_i)-\expec{\xi(f-f^*)}{}}\leq \tau_0\given[\Big]\sup_{j\in\{1,2,\cdots\} }\abs{\xi_j(f-f^*)(X_j)}\leq B\right)\\
	+&\pro\left(\sup_{j\in\{1,2,\cdots\} }\abs{\xi_j(f-f^*)(X_j)}\geq B\right)\\
	\leq& \pro\left(\abs{\frac{1}{N}\sum_{i=1}^N\xi_i(f-f^*)(X_i)-\expec{\xi(f-f^*)}{}}\leq \tau_0\given[\Big]\sup_{j\in\{1,2,\cdots\} }\abs{\xi_j(f-f^*)(X_j)}\leq B\right)
	+p(B)
\end{align*}

Note that, conditioned on the event $\{\sup_{j\in\{1,2,\cdots\} }\abs{\xi_j(f-f^*)(X_j)}\leq B\}$,  $g\left(\{\xi_i\}_{i=1}^N,\{X_i\}_{i=1}^N\right)=\frac{1}{N}\sum_{i=1}^N\xi_i(f-f^*)(X_i)$ is $2B/N$-Lipschitz continuous w.r.t Hamming metric.

because, for some $i \in \{1,2,\cdots,N\}$
\begin{align*}
	&\abs{\phi\left(\{\xi_i\}_{i=1}^N,\{X_i\}_{i=1}^N\right)-\phi\left(\{\xi_i\}_{i=1}^N,X_1,X_2,\cdots,X_{i-1},X_i',X_{i+1},\cdots,X_N\right)}\\
	=&\abs{\frac{1}{N}\xi_i(f-f^*)(X_i)-\frac{1}{N}\xi_i(f-f^*)(X_i')}\leq \frac{2B}{N}
\end{align*}
One gets the same bound if 

Then, conditioned on the event $\{\sup_{j\in\{1,2,\cdots\} }\abs{\xi_j(f-f^*)(X_j)}\leq B\}$, using Theorem 9 of \cite{36944}, we have,
\begin{align}
	\pro\left(\abs{\frac{1}{N}\sum_{i=1}^N\xi_i(f-f^*)(X_i)-\expec{\xi(f-f^*)}{}}\geq \tau_0\right)\leq 2\exp\left(-\frac{N\tau_0^2}{2B^2\left(1+2\sum_{i=1}^{N}\phi(i)\right)^2}\right) \numberthis\label{eq:noiseboundeddiff}
\end{align}
\fi
Combining \eqref{eq:PnLfintermedbound}, and \eqref{eq:noiseconc}, with probability at least $\mathscr{P}_1-\mathscr{P}_2$, for every $f\in \cF$ that satisfies $\|f-f^*\|_{L_2}\geq \rho$, we get 
\begin{align*}
	P_NL_f\geq -2\tau_0+\frac{\tau^2\|f-f^*\|^2_{L_2}Q_\cH(2\tau)}{4}
\end{align*}
Choosing $\tau_0=\frac{\tau^2\|f-f^*\|^2_{L_2}Q_\cH(2\tau)}{16}>\frac{\tau^2\omega_\mu^2(\cH,\tau Q_{\cF-\cF}(2\tau)/16)Q_\cH(2\tau)}{16}:=\tau^*$, we have, $$P_NL_f>0.$$ But the empirical minimizer $\hat{f}$ satisfies $P_NL_{\hat{f}}\leq 0$. This implies that with probability at least $\mathscr{P}$,
\begin{align*}
	\|\hat{f}-f^*\|\leq\rho
\end{align*}
where $\mathscr{P}$ is given by
\begin{align*}
	\mathscr{P}=&1-2\exp\left(-\frac{NQ_\cH(2\tau)^3}{2(4-Q_\cH(2\tau))^2}\left(\frac{c}{\mathscr{G}(N)}\right)^\frac{1}{\eta_1}\right)-\frac{NQ_\cH(2\tau)c^\frac{1}{\eta_1}}{4\mathscr{G}(N)^\frac{1}{\eta_1}}\exp(-\mathscr{G}(N))\\
	-&N\exp\left(-\frac{(N\tau^*)^\eta}{C_1}\right)-\exp\left(-\frac{N^2{\tau^*}^2}{C_2(1+NV)}\right)-\exp\left(-\frac{N{\tau^*}^2}{C_3}\exp\left(\frac{(N\tau^*)^{\eta(1-\eta)}}{C_4(\log (N\tau^*))^\eta}\right)\right)
\end{align*}
\end{proof} 
\fi



\iffalse
\textbf{Note on high probability bound on $|f-f^*|$:}
Let the small-ball condition hold for $u=u_0$ with small-ball probability $Q_\cH(u_0)$. We have, for any $B>0$,
\begin{align}
	\expec{|h(x)|^2}{}=&\int_{|h(x)|<B}|h(x)|^2 dP(x)+\int_{|h(x)|\geq B}|h(x)|^2 dP(x)\\
	\geq & \int_{|h(x)|\geq B}|h(x)|^2 dP(x)\\
	=&B^\pro(|h(x)|\geq B)
\end{align}
Since, $\expec{|h(x)|^2}{}\leq\alpha_N^2$, we have, $B^\pro(|h(x)|\geq B)\leq \alpha_N^2$ for all $B>0$. Setting, $B=u_0\sqrt{\expec{|h(x)|^2}{}}$, using small-ball condition we have,
\begin{align}
	&u_0^2\expec{|h(x)|^2}{}\pro\left(|h(x)|\geq u_0\sqrt{\expec{|h(x)|^2}{}}\right)\leq \alpha_N^2\\
	&u_0^2\expec{|h(x)|^2}{}Q_\cH(u_0)\leq \alpha_N^2\\
	&u_0\leq \frac{\alpha_N}{\sqrt{\expec{|h(x)|^2}{}Q_\cH(u_0)}}:=u_1
\end{align}
Then $\pro\left(|h(x)|\geq u_1\sqrt{\expec{|h(x)|^2}{}}\right)\leq Q_\cH(u_0)$, i.e., $\pro\left(|h(x)|\leq \frac{\alpha_N}{\sqrt{Q_\cH(u_0)}}\right)\geq 1-Q_\cH(u_0)$.
\textcolor{}{Is something better possible? Also, still need a bound on $\xi_i$.}\\
We also have from small-ball condition $\pro\left(|h(x)|\geq u_0\sqrt{\expec{|h(x)|^2}{}}\right)\geq Q_\cH(u_0)$. 
\fi
\iffalse
{\color{red}
Probably the argument below can be used for the above purpose but I need to think more:}
Let $W_i=\xi_iX_i, i=1,2,\cdots,N$ be a sequence of $\iid$ variables which are independent versions of the random variable $W$. If $W$ has polynomially decaying tail, i.e., if $W$ has finite $L_p$ norms only for $2\leq p \leq p_0$, then $\bar{W}=N^{-1}\sum_{i=1}^NW_i$ has finite $L_p$ norm for $2\leq p \leq p_0$ as,
\begin{align*}
	\|\bar{W}\|_{L_p}\leq N^{-1}\sum_{i=1}^N\|W_i\|_{L_p}<\infty
\end{align*}
Also, $\bar{W}$ cannot have finite $L_p$ norm for $p>p_0$ since, for $p>p_0$
\begin{align*}
	\|\bar{W}\|_{L_p}=\frac{1}{N}\left(\expec{\sum_{i=1}^NW_i^p+R_W}{}\right)^\frac{1}{p}
\end{align*}
for some $R_W>0$. But $\expec{W_i^p}{}$ does not exist. So $\|\bar{W}\|_{L_p}$ has a similar tail behavior as $W$. To know the exact constant of the tail decay (which may depend on $N$) we can use a finite order $z$-transform of $G_W(z)$ to get the z-transform of $\bar{W}$ which will be $G_{W/N}(z)^N$. Not sure what this will lead to yet. 
\fi


\iffalse
\newpage
\section{Notes}
{\color{red}
	\begin{enumerate}
		\iffalse
		\item Assuming bound on $\xi_i$ and $(f-f^*)(X_i)$ is not enough. Since the sequence is dependent we need the joint mass to be concentrated in a bounded region which may not be very restrictive compared to the original setting. A similar kind of assumption could be to assume the existence of a constant $\alpha_{b\mu}(\gamma,\delta)$ where $b\mu$ is the size of the block that is being removed.
		\item Is it possible to get a bound on $\left( \frac{1}{N}\sum_{i=1}^N\xi_i(f-f^*)(X_i)-\expec{\xi(f-f^*)}{}\right)$ writing it as a sum of Martingale difference sequence, and using the property that it is a stationary sequence? So far I have only found results for bounded sequence. 
		\fi
		\item Explore the Bernoulli contraction technique for the noise part. 
		\item Here there is a dependence between $\tau_0$ and $\|f-f*\|_{L_2}$ unlike \cite{pmlr-v35-mendelson14}, since they assume that there is no dependence between $\gamma$ and $\delta$. In other words, if one wants to get a high probability result from the bounds in \cite{pmlr-v35-mendelson14}, one has to get a meaningful $\alpha_N(\gamma,\delta)$ for small $\delta$ which does not depend on $\gamma$. For us, this is not true (that is there is dependence between $\tau_0$ and $p(B)$) since we are using concentration inequality instead of assuming an existence of a suitable $\alpha_N(\gamma,\delta)$. Below I am providing another version of this result which is more similar to the result in \cite{pmlr-v35-mendelson14}. 
		\item We may need to think about the horizon over which we are interested in the generalization error, since the bounds on the sup of multiplier process depends on that.
		\item We need consider test point which depends on the training sample. 
		\item Check if marginally-weibull is enough (not that important).
		\item What happens when the coordinates are not independent in the examples.  
\end{enumerate}}
\fi
